The rigidity problem for analytic critical circle maps

It is shown that if $f$ and $g$ are any two analytic critical circle mappings with the same irrational rotation number, then the conjugacy that maps the critical point of $f$ to that of $g$ has regularity $C^{1+\alpha}$ at the critical point, with a universal value of $\alpha>0$. As a consequence, a new proof of the hyperbolicity of the full renormalization horseshoe of critical circle maps is given.

==> figpic/holpair <==
#FIG 3.2
Landscape
Center
Inches
Letter  
10.00
Single
-2
1200 2
0 32 #c6b797
0 33 #eff8ff
0 34 #dccba6
0 35 #404040
0 36 #808080
0 37 #c0c0c0
0 38 #e0e0e0
0 39 #8e8f8e
0 40 #aaaaaa
0 41 #555555
0 42 #bebebe
0 43 #515151
0 44 #e7e3e7
0 45 #000049
0 46 #797979
0 47 #303430
0 48 #414141
0 49 #c7b696
0 50 #8e8e8e
0 51 #414541
0 52 #8e8e8e
0 53 #000079
0 54 #ff8200
0 55 #007d00
0 56 #0000be
0 57 #444444
0 58 #cccccc
0 59 #fff2d3
0 60 #ffe4ae
0 61 #ffd279
0 62 #cfcfcf
0 63 #999999
0 64 #b2b2b2
0 65 #868286
0 66 #c7c3c7
0 67 #868686
0 68 #c7c7c7
0 69 #e7e7e7
0 70 #f7f7f7
0 71 #9e9e9e
0 72 #717571
0 73 #effbff
0 74 #666666
0 75 #e2e2ee
0 76 #94949a
0 77 #dbdbdb
0 78 #a1a1b7
0 79 #9c0000
0 80 #ededed
0 81 #86acff
0 82 #7070ff
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6093.020 1531.365 6255 1847 6039 1882 5891 1823
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 5653.504 1259.771 5891 1823 5659 1871 5444 1834
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 5159.806 1547.535 5444 1834 5269 1936 5066 1940
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 5933.350 2654.151 5884 2554 6015 2578 6045 2654
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6077.614 2926.840 6050 2654 6195 2679 6282 2744
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6487.804 2869.030 6282 2744 6397 2646 6517 2630
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6631.840 2546.102 6517 2630 6527 2450 6626 2404
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6669.529 2269.957 6626 2404 6533 2235 6615 2140
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 6603.529 1787.600 6623 2137 6372 2050 6258 1843
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 2952.483 2514.974 3063 2417 3068 2607 2993 2657
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3018.000 2157.000 3068 2407 3208 2327 3268 2207
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3394.961 2020.976 3273 2207 3448 2237 3543 2187
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3895.827 1801.509 3548 2177 3683 2267 4003 2302
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 2882.812 2809.287 2988 2657 3063 2767 3043 2902
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3160.909 2997.147 3048 2902 3188 2852 3303 2957
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3396.306 3008.210 3308 2957 3383 2907 3478 2947
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3554.475 2951.836 3478 2947 3538 2877 3608 2897
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3659.563 2912.680 3608 2902 3693 2872 3688 2957
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3700.321 3002.893 3688 2957 3743 2982 3718 3047
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6093.020 4572.635 6255 4257 6039 4222 5891 4281
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 5653.504 4844.229 5891 4281 5659 4233 5444 4270
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 5159.806 4556.465 5444 4270 5269 4168 5066 4164
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 5933.350 3449.849 5884 3550 6015 3526 6045 3450
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6077.614 3177.160 6050 3450 6195 3425 6282 3360
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6487.804 3234.970 6282 3360 6397 3458 6517 3474
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6631.840 3557.898 6517 3474 6527 3654 6626 3700
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6669.529 3834.043 6626 3700 6533 3869 6615 3964
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 6603.529 4316.400 6623 3967 6372 4054 6258 4261
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 2952.483 3589.026 3063 3687 3068 3497 2993 3447
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3018.000 3947.000 3068 3697 3208 3777 3268 3897
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3394.961 4083.024 3273 3897 3448 3867 3543 3917
5 1 0 1 0 7 50 0 -1 0.000 0 0 0 0 3895.827 4302.491 3548 3927 3683 3837 4003 3802
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 2882.812 3294.713 2988 3447 3063 3337 3043 3202
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3160.909 3106.853 3048 3202 3188 3252 3303 3147
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3396.306 3095.790 3308 3147 3383 3197 3478 3157
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3554.475 3152.164 3478 3157 3538 3227 3608 3207
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3659.563 3191.320 3608 3202 3693 3232 3688 3147
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 3700.321 3101.107 3688 3147 3743 3122 3718 3057
5 1 1 1 0 7 50 0 -1 4.000 0 0 1 0 3666.575 2117.524 3466 2407 3316 2084 3616 1769
	2 1 1.00 60.00 120.00
5 1 1 1 0 7 50 0 -1 4.000 0 1 1 0 5469.882 2030.926 5851 2242 5889 1912 5431 1597
	2 1 1.00 60.00 120.00
5 1 1 1 0 7 50 0 -1 4.000 0 1 1 0 4469.599 2325.865 4576 2549 4659 2167 4224 2354
	2 1 1.00 60.00 120.00
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4433 3052 595 595 4433 3052 4448 2457
1 1 0 1 0 7 50 0 -1 0.000 1 0.0000 4880 3042 2963 1755 4880 3042 7843 4797
2 1 0 1 -1 -1 10 0 -1 0.000 0 0 0 0 0 2
	 2393 3052 7235 3053
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5064 1941 4425 3048
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4433 3052 3998 2302
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5064 4163 4425 3056
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4433 3052 3998 3802
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3728 3052 5563 3052
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5881 2551 5786 2502 5702 2551
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5704 2551 5585 2552 5587 2657
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5592 2660 5515 2715 5551 2807
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5557 2810 5502 2898 5554 3049
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5881 3553 5786 3602 5702 3553
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5704 3553 5585 3552 5587 3447
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5592 3444 5515 3389 5551 3297
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 3
	 5557 3294 5502 3206 5554 3055
	 0.000 -1.000 0.000
4 1 0 50 0 0 12 0.0000 4 120 135 4408 2722 D\001
4 1 0 50 0 0 12 0.0000 4 120 135 3378 2647 V\001
4 1 0 50 0 0 12 0.0000 4 120 135 5433 2372 U\001
4 1 0 50 0 0 12 0.0000 4 120 375 7153 2659 Delta\001
4 2 0 50 0 0 12 0.0000 4 120 135 3241 2077 xi\001
4 0 0 50 0 0 12 0.0000 4 105 195 5881 1702 eta\001
4 1 0 50 0 0 12 0.0000 4 120 585 4479 1942 xicirceta\001
4 1 0 50 0 0 12 0.0000 4 120 90 4419 3322 0\001


==> figpic/makefile <==
clean:
	rm -f *~ *.aux *.log \#*\# *.dvi *.toc *.blg *.bak
cleanall: clean


==> pic/makefile <==
all: picxfig.gpl
	./pic.pl
clean:
	rm -f *~ *.aux *.log \#*\# *.dvi *.toc *.blg
cleanall: clean
	rm -f gnudat/*


==> picparab/makefile <==
all: pic.fig picxfig.gpl

pic.fig:picxfig.gpl
	gnuplot picxfig.gpl
picxfig.gpl:pic.pl
	./pic.pl
clean:
	rm -f *~ *.aux *.log \#*\# *.dvi *.toc *.blg
cleanall: clean
	rm -f gnudat/*

